Can a calibration metric be both testable and actionable?

Forecast probabilities often serve as critical inputs for binary decision making. In such settings, calibration$\unicode{x2014}$ensuring forecasted probabilities match empirical frequencies$\unicode{x2014}$is essential. Although the common notion of Expected Calibration Error (ECE) provides actionable insights for decision making, it is not testable: it cannot be empirically estimated in many practical cases. Conversely, the recently proposed Distance from Calibration (dCE) is testable, but it is not actionable since it lacks decision-theoretic guarantees needed for high-stakes applications. To resolve this question, we consider Cutoff Calibration Error, a calibration measure that bridges this gap by assessing calibration over intervals of forecasted probabilities. We show that Cutoff Calibration Error is both testable and actionable, and we examine its implications for popular post-hoc calibration methods, such as isotonic regression and Platt scaling.

==> src/existing-measure.tex <==
\section{Existing measures of calibration}

For the ensuing overview of existing definitions of measures of calibration, we will assume the more general setting that $Y \in [0,1]$, since all of our guarantees will hold in this more general setting. Existing calibration literature frequently focuses just on the binary $Y$ setting.

\begin{definition}
    Suppose $Y \in [0,1]$ is a random variable and $f: \mathcal{X} \rightarrow [0,1]$ is a probability forecast for event $Y$ using random covariates $X \in \mathcal{X}$. Then, $f$ is \textbf{perfectly calibrated} if 
\begin{equation}
    \mathbb E[Y\mid f(X)] = f(X) \text{ a.s.}
\end{equation}
\end{definition}

We cannot guarantee perfect calibration to hold outside of very simple choices for the forecast model $f$, which motivates the need to measure deviation from perfect calibration. A natural relaxation of perfect calibration is as follows.

\begin{definition}
    The \textbf{Expected Calibration Error (\ece)} is
\begin{equation}
        \ecem(f):= \mathbb{E}\left|\mathbb{E}[Y \mid f(X)]-f(X)\right|
\end{equation}
\end{definition}



\todo{Add a footnote explaining that for data-driven $\hat{f}_n$ we measure $\Delta_{\text{ECE}}(\hat{f}_n)$}

\citet{blasiok2023unifying} propose an alternate measure of calibration, \dce, which measures calibration of $f$ as how close $f$ is to any function $g$ that is perfectly calibrated.
\begin{definition}
    The \textbf{Distance from Calibration (dCE)} of a function $f$ is:
    \begin{equation}
        \dcem(f) := \inf_{\substack{g: \mathcal{X} \rightarrow [0,1]:\\ \mathbb{E}[Y \mid g(X)]=g(X)}}  \mathbb{E}|g(X)-f(X)|
\end{equation}  
\end{definition}

The ECE and dCE measures of calibration error can be related as follows: \becca{put in sentence}
\begin{proposition}[{\citet[Lemma 4.7]{blasiok2023unifying}}]\label{prop:dCE_vs_ECE}
    For any function $f:\cX\to[0,1]$,
    \[\dcem(f) \leq \ecem(f).\]\label{prop:ece_dce_ineq}
\end{proposition}

An umbrella notation that we can use to bridge dCE and ECE is Weighted Calibration Error, introduced by \citet{gopalan2022low}, which built on existing work \citep{kim2019multiaccuracy, hebert2018multicalibration, kakade2008deterministic}.

\begin{definition}
    Let $\mathcal{C} \subseteq [-1,1]^{f(\mathcal{X})}$. Then, \textbf{Weighted Calibration Error} is the following:
    \begin{equation}
\Delta_{\operatorname{wCE}}(f; \mathcal{C}) := \sup_{w \in \mathcal{C}} \mathbb E [w(f(X))(Y - f(X))].
\end{equation}
\end{definition} 
We can now relate Weighted Calibration Error to \ece and \dce.
When $\mathcal{L}_1$ is the class of all 1-Lipschitz functions, \citet{blasiok2023unifying} show 
\begin{equation}
    \dcem(f)^2 / 8 \leq \Delta_{\operatorname{wCE}}(f; \mathcal{L}_1) \leq 2 \cdot \dcem(f).
\end{equation}
In addition, when we let $C$ include any measurable function that outputs in $[-1,1]$, we get
\begin{equation}
\Delta_{\operatorname{wCE}}(f; [-1,1]^{f(\mathcal{X})}) = \ecem(f).\label{eq:ece_wce}
\end{equation}


